Transportation Technology and Gentrification: Evidence from the entry of Ridesharing Services

We analyze the staggered entry of rideshare services across U.S. metropolitan areas, estimating its effect on the spatial redistribution and real outcomes of residents. Ridesharing services gentrify urban areas-especially those with ex-ante lower housing values-causing housing prices to rise 9 percent, with the in-migration of rich-younger individuals more than offsetting the out-migration of incumbent residents and reduced in-migration of poorer individuals. Impact on incumbent residents is conditional on ex-ante homeownership. For homeowners, there is no displacement and a decline in delinquency rates. For non-homeowners, displacement and delinquency rates rise 11 percent and 42 percent, respectively. Our study emphasizes how the private provision of high-end transportation technologies can increase urbanization and exacerbate inequality.

==> tables/A11_Entry_pooling_zipcodes.tex <==
\begin{tabular}{lcccc}
	\toprule
	\toprule
	& House Price Index$_{z,y}$ & Rental Prices$_{z,y}$ & Vacancy Rate$_{z,y}$ & Number of Vacancies$_{z,y}$ \\
	& (1)            & (2)            & (3)            & (4) \\
	\midrule
	&                &                &                &  \\
	PreEntry 2-Years & -0.020         & 0.001          & -0.159         & 0.001 \\
	& (0.021)        & (0.004)        & (0.102)        & (0.009) \\
	PreEntry 1-Years & -0.014         & 0.007          & -0.161         & -0.003 \\
	& (0.021)        & (0.006)        & (0.113)        & (0.009) \\
	PostEntry 0-Years & 0.008***       & 0.007*         & -0.303***      & -0.011** \\
	& (0.002)        & (0.004)        & (0.057)        & (0.005) \\
	PostEntry 1-Years & 0.013***       & 0.014***       & -0.823***      & -0.029*** \\
	& (0.003)        & (0.004)        & (0.073)        & (0.005) \\
	PostEntry 2-Years & 0.023***       & 0.022***       & -0.685***      & -0.035*** \\
	& (0.003)        & (0.005)        & (0.083)        & (0.007) \\
	PostEntry 3-Years & 0.035***       & 0.024***       & -0.626***      & -0.041*** \\
	& (0.004)        & (0.006)        & (0.108)        & (0.008) \\
	PostEntry 4-Years & 0.045***       & 0.029***       & -0.583***      & -0.054*** \\
	& (0.004)        & (0.007)        & (0.142)        & (0.009) \\
	&                &                &                &  \\
	Observations   & 31,210         & 33,254         & 30,813         & 30,813 \\
	Zip-code FE     & Yes            & Yes            & Yes            & Yes \\
	MSA-Year FE    & Yes            & Yes            & Yes            & Yes \\
	Average Dep. Variable & 5              & 7.4            & 2.9            & 8.9 \\
	\bottomrule
\end{tabular}%

==> tables/AX_Entry_rideshare_individuals.tex <==
\begin{tabular}{lcccccc}
	\toprule
	\toprule
	\multicolumn{1}{r}{} & \multicolumn{2}{c}{\#Movers into Zip-code$_{z,y}$} & \multicolumn{2}{c}{\#Movers into Zip-code same MSA$_{z,y}$} & \multicolumn{2}{c}{\#Movers into Zip-code other MSA$_{z,y}$} \\
	\multicolumn{1}{r}{} & \multicolumn{1}{c}{(1)} & \multicolumn{1}{c}{(2)} & \multicolumn{1}{c}{(3)} & \multicolumn{1}{c}{(4)} & \multicolumn{1}{c}{(5)} & \multicolumn{1}{c}{(6)} \\
	\midrule
	\multicolumn{1}{r}{} &                &                &                &                &                &  \\
	PreEntry 2-Years & \multicolumn{1}{c}{0.002} & \multicolumn{1}{c}{0.007} & \multicolumn{1}{c}{-0.005} & \multicolumn{1}{c}{0.042**} & \multicolumn{1}{c}{-0.022} & \multicolumn{1}{c}{-0.018} \\
	\multicolumn{1}{r}{} & \multicolumn{1}{c}{(0.020)} & \multicolumn{1}{c}{(0.015)} & \multicolumn{1}{c}{(0.026)} & \multicolumn{1}{c}{(0.020)} & \multicolumn{1}{c}{(0.033)} & \multicolumn{1}{c}{(0.020)} \\
	PostEntry 1-Years & \multicolumn{1}{c}{0.011} & \multicolumn{1}{c}{0.019} & \multicolumn{1}{c}{-0.043} & \multicolumn{1}{c}{0.061**} & \multicolumn{1}{c}{0.030} & \multicolumn{1}{c}{-0.020} \\
	\multicolumn{1}{r}{} & \multicolumn{1}{c}{(0.029)} & \multicolumn{1}{c}{(0.021)} & \multicolumn{1}{c}{(0.037)} & \multicolumn{1}{c}{(0.028)} & \multicolumn{1}{c}{(0.047)} & \multicolumn{1}{c}{(0.028)} \\
	PostEntry 0-Years & \multicolumn{1}{c}{0.032} & \multicolumn{1}{c}{0.047***} & \multicolumn{1}{c}{0.023} & \multicolumn{1}{c}{0.031} & \multicolumn{1}{c}{0.059**} & \multicolumn{1}{c}{0.012} \\
	\multicolumn{1}{r}{} & \multicolumn{1}{c}{(0.024)} & \multicolumn{1}{c}{(0.017)} & \multicolumn{1}{c}{(0.026)} & \multicolumn{1}{c}{(0.027)} & \multicolumn{1}{c}{(0.026)} & \multicolumn{1}{c}{(0.019)} \\
	PostEntry 1-Years & \multicolumn{1}{c}{0.078***} & \multicolumn{1}{c}{0.041*} & \multicolumn{1}{c}{0.039*} & \multicolumn{1}{c}{0.105***} & \multicolumn{1}{c}{0.103***} & \multicolumn{1}{c}{-0.020} \\
	\multicolumn{1}{r}{} & \multicolumn{1}{c}{(0.020)} & \multicolumn{1}{c}{(0.021)} & \multicolumn{1}{c}{(0.023)} & \multicolumn{1}{c}{(0.025)} & \multicolumn{1}{c}{(0.027)} & \multicolumn{1}{c}{(0.023)} \\
	PostEntry 2-Years & \multicolumn{1}{c}{0.175***} & \multicolumn{1}{c}{0.077***} & \multicolumn{1}{c}{0.243***} & \multicolumn{1}{c}{0.121***} & \multicolumn{1}{c}{0.165***} & \multicolumn{1}{c}{0.030} \\
	\multicolumn{1}{r}{} & \multicolumn{1}{c}{(0.020)} & \multicolumn{1}{c}{(0.024)} & \multicolumn{1}{c}{(0.025)} & \multicolumn{1}{c}{(0.041)} & \multicolumn{1}{c}{(0.029)} & \multicolumn{1}{c}{(0.027)} \\
	PostEntry 3-Years & \multicolumn{1}{c}{0.261***} & \multicolumn{1}{c}{0.023} & \multicolumn{1}{c}{0.102***} & \multicolumn{1}{c}{0.116***} & \multicolumn{1}{c}{0.431***} & \multicolumn{1}{c}{-0.032} \\
	\multicolumn{1}{r}{} & \multicolumn{1}{c}{(0.024)} & \multicolumn{1}{c}{(0.027)} & \multicolumn{1}{c}{(0.027)} & \multicolumn{1}{c}{(0.029)} & \multicolumn{1}{c}{(0.033)} & \multicolumn{1}{c}{(0.036)} \\
	PostEntry 4-Years & \multicolumn{1}{c}{0.287***} & \multicolumn{1}{c}{0.019} & \multicolumn{1}{c}{0.389***} & \multicolumn{1}{c}{0.149***} & \multicolumn{1}{c}{0.173***} & \multicolumn{1}{c}{-0.071**} \\
	\multicolumn{1}{r}{} & \multicolumn{1}{c}{(0.024)} & \multicolumn{1}{c}{(0.027)} & \multicolumn{1}{c}{(0.029)} & \multicolumn{1}{c}{(0.043)} & \multicolumn{1}{c}{(0.031)} & \multicolumn{1}{c}{(0.033)} \\
	\multicolumn{1}{r}{} &                &                &                &                &                &  \\
	Observations   & 8,707          & 15,952         & 8,707          & 15,952         & 8,707          & 15,952 \\
	Zip-code FE     & \multicolumn{1}{c}{Yes} & \multicolumn{1}{c}{Yes} & \multicolumn{1}{c}{Yes} & \multicolumn{1}{c}{Yes} & \multicolumn{1}{c}{Yes} & \multicolumn{1}{c}{Yes} \\
	State-Year FE  & \multicolumn{1}{c}{Yes} & \multicolumn{1}{c}{Yes} & \multicolumn{1}{c}{Yes} & \multicolumn{1}{c}{Yes} & \multicolumn{1}{c}{Yes} & \multicolumn{1}{c}{Yes} \\
	Zip-codes       & \multicolumn{1}{c}{Urban} & \multicolumn{1}{c}{Suburban} & \multicolumn{1}{c}{Urban} & \multicolumn{1}{c}{Suburban} & \multicolumn{1}{c}{Urban} & \multicolumn{1}{c}{Suburban} \\
	Average Dep. Variable & 3.7            & 3.2            & 3.3            & 2.8            & 2.4            & 2.2 \\
	\bottomrule
\end{tabular}%

==> tables/IA_Entry_mortgage_characteristics_commented_out_.tex <==
\begin{tabular}{lcccccc}
	\toprule
	\toprule
	\multicolumn{1}{r}{} & \multicolumn{2}{c}{Minority$_{i,y}$} & \multicolumn{2}{c}{Not-Owner-Occupied$_{i,y}$} & \multicolumn{2}{c}{Mortgage Value$_{i,y}$}  \\
	\multicolumn{1}{r}{} & \multicolumn{1}{c}{(1)} & \multicolumn{1}{c}{(2)} & \multicolumn{1}{c}{(3)} & \multicolumn{1}{c}{(4)} & \multicolumn{1}{c}{(5)} & \multicolumn{1}{c}{(6)}  \\
	\midrule
	\multicolumn{1}{r}{} &                &                &                &                &                &                 \\
	PreEntry 2-Years & \multicolumn{1}{c}{0.001} & \multicolumn{1}{c}{-0.002} & \multicolumn{1}{c}{0.001} & \multicolumn{1}{c}{-0.002} & \multicolumn{1}{c}{-0.009**} & \multicolumn{1}{c}{0.001}  \\
	\multicolumn{1}{r}{} & \multicolumn{1}{c}{(0.002)} & \multicolumn{1}{c}{(0.002)} & \multicolumn{1}{c}{(0.005)} & \multicolumn{1}{c}{(0.009)} & \multicolumn{1}{c}{(0.005)} & \multicolumn{1}{c}{(0.005)}  \\
	PostEntry 1-Years & \multicolumn{1}{c}{-0.000} & \multicolumn{1}{c}{0.002} & \multicolumn{1}{c}{-0.005} & \multicolumn{1}{c}{-0.018} & \multicolumn{1}{c}{-0.025***} & \multicolumn{1}{c}{-0.005}  \\
	\multicolumn{1}{r}{} & \multicolumn{1}{c}{(0.003)} & \multicolumn{1}{c}{(0.003)} & \multicolumn{1}{c}{(0.008)} & \multicolumn{1}{c}{(0.012)} & \multicolumn{1}{c}{(0.007)} & \multicolumn{1}{c}{(0.008)}  \\
	PostEntry 0-Years & \multicolumn{1}{c}{-0.000} & \multicolumn{1}{c}{0.006***} & \multicolumn{1}{c}{0.001} & \multicolumn{1}{c}{-0.020***} & \multicolumn{1}{c}{-0.016***} & \multicolumn{1}{c}{0.001} \\
	\multicolumn{1}{r}{} & \multicolumn{1}{c}{(0.002)} & \multicolumn{1}{c}{(0.002)} & \multicolumn{1}{c}{(0.006)} & \multicolumn{1}{c}{(0.007)} & \multicolumn{1}{c}{(0.005)} & \multicolumn{1}{c}{(0.006)}  \\
	PostEntry 1-Years & \multicolumn{1}{c}{-0.002} & \multicolumn{1}{c}{0.011***} & \multicolumn{1}{c}{0.009*} & \multicolumn{1}{c}{-0.034***} & \multicolumn{1}{c}{-0.012**} & \multicolumn{1}{c}{0.009*}  \\
	\multicolumn{1}{r}{} & \multicolumn{1}{c}{(0.003)} & \multicolumn{1}{c}{(0.003)} & \multicolumn{1}{c}{(0.006)} & \multicolumn{1}{c}{(0.007)} & \multicolumn{1}{c}{(0.006)} & \multicolumn{1}{c}{(0.006)}  \\
	PostEntry 2-Years & \multicolumn{1}{c}{-0.005} & \multicolumn{1}{c}{0.020***} & \multicolumn{1}{c}{0.013*} & \multicolumn{1}{c}{-0.075***} & \multicolumn{1}{c}{-0.024***} & \multicolumn{1}{c}{0.013*}  \\
	\multicolumn{1}{r}{} & \multicolumn{1}{c}{(0.005)} & \multicolumn{1}{c}{(0.004)} & \multicolumn{1}{c}{(0.006)} & \multicolumn{1}{c}{(0.016)} & \multicolumn{1}{c}{(0.008)} & \multicolumn{1}{c}{(0.006)}  \\
	PostEntry 3-Years & \multicolumn{1}{c}{0.000} & \multicolumn{1}{c}{0.026***} & \multicolumn{1}{c}{0.014*} & \multicolumn{1}{c}{-0.108***} & \multicolumn{1}{c}{-0.029***} & \multicolumn{1}{c}{0.014*}  \\
	\multicolumn{1}{r}{} & \multicolumn{1}{c}{(0.006)} & \multicolumn{1}{c}{(0.005)} & \multicolumn{1}{c}{(0.008)} & \multicolumn{1}{c}{(0.013)} & \multicolumn{1}{c}{(0.010)} & \multicolumn{1}{c}{(0.008)} \\
	PostEntry 4-Years & \multicolumn{1}{c}{-0.006} & \multicolumn{1}{c}{0.038***} & \multicolumn{1}{c}{0.021**} & \multicolumn{1}{c}{-0.085***} & \multicolumn{1}{c}{-0.031**} & \multicolumn{1}{c}{0.021**}  \\
	\multicolumn{1}{r}{} & \multicolumn{1}{c}{(0.008)} & \multicolumn{1}{c}{(0.006)} & \multicolumn{1}{c}{(0.010)} & \multicolumn{1}{c}{(0.016)} & \multicolumn{1}{c}{(0.012)} & \multicolumn{1}{c}{(0.010)}  \\
	\multicolumn{1}{r}{} &                &                &                &                &                &              \\
	Observations   & 2,096,925      & 3,222,277      & 2,295,577      & 3,534,990      & 2,295,577      & 3,534,990       \\
	MSA FE         & \multicolumn{1}{c}{Yes} & \multicolumn{1}{c}{Yes} & \multicolumn{1}{c}{Yes} & \multicolumn{1}{c}{Yes} & \multicolumn{1}{c}{Yes} & \multicolumn{1}{c}{Yes} \\
	State-Year FE  & \multicolumn{1}{c}{Yes} & \multicolumn{1}{c}{Yes} & \multicolumn{1}{c}{Yes} & \multicolumn{1}{c}{Yes} & \multicolumn{1}{c}{Yes} & \multicolumn{1}{c}{Yes}  \\
	Zip-codes       & \multicolumn{1}{c}{Urban} & \multicolumn{1}{c}{Suburban} & \multicolumn{1}{c}{Urban} & \multicolumn{1}{c}{Suburban} & \multicolumn{1}{c}{Suburban} & \multicolumn{1}{c}{Urban}  \\
	Avg. Dep. Variable & 0.41           & 0.25           & 0.12           & 0.07           & 5.3            & 5.4           \\
	\bottomrule
\end{tabular}%

==> tables/IA_Entry_mortgage_origination_commented_out_.tex <==
\begin{tabular}{lcccc}
	\toprule
	\toprule
	\multicolumn{1}{r}{} & \multicolumn{1}{c}{Minority$_{i,y}$} & \multicolumn{1}{c}{Non-Owner-Occupied$_{i,y}$} & \multicolumn{1}{c}{Mortgage Value$_{i,y}$} & \multicolumn{1}{c}{Home Value$_{i,y}$} \\
	\multicolumn{1}{r}{} & \multicolumn{1}{c}{(1)} & \multicolumn{1}{c}{(2)} & \multicolumn{1}{c}{(3)} & \multicolumn{1}{c}{(4)} \\
	\midrule
	\multicolumn{1}{r}{} &                &                &                &  \\
	PreEntry 2-Years & \multicolumn{1}{c}{0.003} & \multicolumn{1}{c}{0.005} & \multicolumn{1}{c}{-0.011} & \multicolumn{1}{c}{0.0010} \\
	\multicolumn{1}{r}{} & \multicolumn{1}{c}{(0.006)} & \multicolumn{1}{c}{(0.004)} & \multicolumn{1}{c}{(0.009)} & \multicolumn{1}{c}{(0.006)} \\
	PostEntry 1-Years & \multicolumn{1}{c}{-0.004} & \multicolumn{1}{c}{0.004} & \multicolumn{1}{c}{0.001} & \multicolumn{1}{c}{0.007} \\
	\multicolumn{1}{r}{} & \multicolumn{1}{c}{(0.007)} & \multicolumn{1}{c}{(0.004)} & \multicolumn{1}{c}{(0.009)} & \multicolumn{1}{c}{(0.006)} \\
	PostEntry 0-Years & \multicolumn{1}{c}{-0.008*} & \multicolumn{1}{c}{-0.002} & \multicolumn{1}{c}{0.015**} & \multicolumn{1}{c}{0.001} \\
	\multicolumn{1}{r}{} & \multicolumn{1}{c}{(0.005)} & \multicolumn{1}{c}{(0.003)} & \multicolumn{1}{c}{(0.006)} & \multicolumn{1}{c}{(0.010)} \\
	PostEntry 1-Years & \multicolumn{1}{c}{-0.016**} & \multicolumn{1}{c}{-0.005} & \multicolumn{1}{c}{0.013**} & \multicolumn{1}{c}{0.015**} \\
	\multicolumn{1}{r}{} & \multicolumn{1}{c}{(0.006)} & \multicolumn{1}{c}{(0.003)} & \multicolumn{1}{c}{(0.007)} & \multicolumn{1}{c}{(0.007)} \\
	PostEntry 2-Years & \multicolumn{1}{c}{-0.018***} & \multicolumn{1}{c}{-0.013***} & \multicolumn{1}{c}{0.031***} & \multicolumn{1}{c}{0.031***} \\
	\multicolumn{1}{r}{} & \multicolumn{1}{c}{(0.006)} & \multicolumn{1}{c}{(0.004)} & \multicolumn{1}{c}{(0.008)} & \multicolumn{1}{c}{(0.005)} \\
	PostEntry 3-Years & \multicolumn{1}{c}{-0.015**} & \multicolumn{1}{c}{-0.012***} & \multicolumn{1}{c}{0.040***} & \multicolumn{1}{c}{0.044***} \\
	\multicolumn{1}{r}{} & \multicolumn{1}{c}{(0.008)} & \multicolumn{1}{c}{(0.004)} & \multicolumn{1}{c}{(0.009)} & \multicolumn{1}{c}{(0.006)} \\
	PostEntry 4-Years & \multicolumn{1}{c}{-0.021***} & \multicolumn{1}{c}{-0.015***} & \multicolumn{1}{c}{0.058***} & \multicolumn{1}{c}{0.073***} \\
	\multicolumn{1}{r}{} & \multicolumn{1}{c}{(0.007)} & \multicolumn{1}{c}{(0.004)} & \multicolumn{1}{c}{(0.010)} & \multicolumn{1}{c}{(0.014)} \\
	\multicolumn{1}{r}{} &                &                &                &  \\
	Observations   & 7,125,352      & 7,804,222      & 7,804,222      & 1,568,432 \\
	Zip-code FE     & \multicolumn{1}{c}{Yes} & \multicolumn{1}{c}{Yes} & \multicolumn{1}{c}{Yes} & \multicolumn{1}{c}{Yes} \\
	MSA-Year FE    & \multicolumn{1}{c}{Yes} & \multicolumn{1}{c}{Yes} & \multicolumn{1}{c}{Yes} & \multicolumn{1}{c}{Yes} \\
	Avg. Dep. Variable & 0.32           & 0.09           & 5.4            & 5.5 \\
	\bottomrule
\end{tabular}%

==> tables/IA_Entry_mortgage_value_commented_out_.tex <==
\begin{tabular}{lcc}
	\toprule
	\toprule
	\multicolumn{1}{r}{} & \multicolumn{1}{c}{\#Mortgage $Applications_{z,y}$} & \multicolumn{1}{c}{$Approval_{i,y}$} \\
	\multicolumn{1}{r}{} & \multicolumn{1}{c}{(1)} & \multicolumn{1}{c}{(2)} \\
	\midrule
	\multicolumn{1}{r}{} &                &  \\
	\multicolumn{1}{r}{} &                &  \\
	PreEntry 2-Years & \multicolumn{1}{c}{-0.053} & \multicolumn{1}{c}{0.003} \\
	\multicolumn{1}{r}{} & \multicolumn{1}{c}{(0.035)} & \multicolumn{1}{c}{(0.002)} \\
	PostEntry 1-Years & \multicolumn{1}{c}{-0.032} & \multicolumn{1}{c}{0.004**} \\
	\multicolumn{1}{r}{} & \multicolumn{1}{c}{(0.035)} & \multicolumn{1}{c}{(0.002)} \\
	PostEntry 0-Years & \multicolumn{1}{c}{-0.011} & \multicolumn{1}{c}{0.004***} \\
	\multicolumn{1}{r}{} & \multicolumn{1}{c}{(0.012)} & \multicolumn{1}{c}{(0.002)} \\
	PostEntry 1-Years & \multicolumn{1}{c}{0.010} & \multicolumn{1}{c}{0.008***} \\
	\multicolumn{1}{r}{} & \multicolumn{1}{c}{(0.012)} & \multicolumn{1}{c}{(0.002)} \\
	PostEntry 2-Years & \multicolumn{1}{c}{0.044***} & \multicolumn{1}{c}{0.009***} \\
	\multicolumn{1}{r}{} & \multicolumn{1}{c}{(0.013)} & \multicolumn{1}{c}{(0.001)} \\
	PostEntry 3-Years & \multicolumn{1}{c}{0.085***} & \multicolumn{1}{c}{0.015***} \\
	\multicolumn{1}{r}{} & \multicolumn{1}{c}{(0.015)} & \multicolumn{1}{c}{(0.002)} \\
	PostEntry 4-Years & \multicolumn{1}{c}{0.141***} & \multicolumn{1}{c}{0.017***} \\
	\multicolumn{1}{r}{} & \multicolumn{1}{c}{(0.015)} & \multicolumn{1}{c}{(0.002)} \\
	\multicolumn{1}{r}{} &                &  \\
	Observations   & 33,008         & 7,006,236 \\
	Loan Controls  & \multicolumn{1}{c}{No} & \multicolumn{1}{c}{Yes} \\
	Zip-code FE     & \multicolumn{1}{c}{Yes} & \multicolumn{1}{c}{Yes} \\
	MSA-Year FE    & \multicolumn{1}{c}{Yes} & \multicolumn{1}{c}{Yes} \\
	Avg. Dep. Variable & 5.1            & 0.89 \\
	\bottomrule
\end{tabular}%
